Adaptive Outlier Detection for Power MOSFETs Based on Gaussian Process Regression

Outlier detection of semiconductor devices is important since manufacturing variation is inherently inevitable. In order to properly detect outliers, it is necessary to consider the discrepancy from underlying trend. Conventional methods are insufficient as they cannot track spatial changes of the trend}}. This study proposes an adaptive outlier detection using Gaussian process regression (GPR) with Student-t likelihood, which captures a gradual spatial change of characteristic variation. According to the credible interval of the GPR posterior distribution, the devices having excessively large deviations against the underlying trend are detected. The proposed methodology is validated by the experiments using a commercial SiC wafer and simulation.

==> Makefile <==
TEX2PDF = latexmk

MAINFILE = main.tex
MAINTARGET = $(MAINFILE:.tex=.pdf)
SUBFILEDIR = sub
SUBFILES = $(wildcard $(SUBFILEDIR)/*.input_tex)
SUBTARGETS = $(SUBFILES:.input_tex=.pdf)

BIBFILES = $(wildcard *.bib)

FIGDIR = fig
SVGFILES = $(wildcard $(FIGDIR)/*.svg)
PNGFILES = $(wildcard $(FIGDIR)/*.png)
JPGFILES = $(wildcard $(FIGDIR)/*.jpg)
SVG2EPSTARGETS = $(SVGFILES:.svg=.eps)
DEPFILES = $(SVG2EPSTARGETS) $(PNGFILES) $(JPGFILES) $(BIBFILES)

main: $(MAINTARGET)
$(MAINTARGET): $(SUBFILES)

subs: $(SUBTARGETS)

all: main subs

dep: $(DEPFILES)

ifeq ($(findstring 1.,$(shell inkscape -V 2>/dev/null)),)
%.pdf: %.svg
	DISPLAY= inkscape -z -D -A $(abspath $@) $(abspath $<)
%.eps: %.svg
	DISPLAY= inkscape -z -D -A $(abspath $@) $(abspath $<)
else
%.pdf: %.svg
	DISPLAY= inkscape -D -o $(abspath $@) $(abspath $<)
%.eps: %.svg
	DISPLAY= inkscape -D -o $(abspath $@) $(abspath $<)
endif

%.pdf: %.tex $(DEPFILES)
	cd $(dir $<) && \
		$(TEX2PDF) $(notdir $<) && \
		ln -sf .tmp/$(notdir $@)

%.tex: %.input_tex
	sed -n 1,/\begin{document}/p $(MAINFILE) > $@
	cat $< >> $@
	sed -n /\end{document}/,$$$$p $(MAINFILE) >> $@
	# Make main.pdf
	cd `git rev-parse --show-toplevel` && make main

arrange:
	rm -rfv .tmp/* */.tmp/*
	rm -fv $(SVG2PDFTARGETS)

clean: arrange
	rm -fv *.pdf $(SUBFILEDIR)/*.pdf

